Interpretability of Machine Learning Methods Applied to Neuroimaging

Deep learning methods have become very popular for the processing of natural images, and were then successfully adapted to the neuroimaging field. As these methods are non-transparent, interpretability methods are needed to validate them and ensure their reliability. Indeed, it has been shown that deep learning models may obtain high performance even when using irrelevant features, by exploiting biases in the training set. Such undesirable situations can potentially be detected by using interpretability methods. Recently, many methods have been proposed to interpret neural networks. However, this domain is not mature yet. Machine learning users face two major issues when aiming to interpret their models: which method to choose, and how to assess its reliability? Here, we aim at providing answers to these questions by presenting the most common interpretability methods and metrics developed to assess their reliability, as well as their applications and benchmarks in the neuroimaging context. Note that this is not an exhaustive survey: we aimed to focus on the studies which we found to be the most representative and relevant.

==> Interpretability Chapter/studies_table.tex <==
\afterpage{%
\clearpage% Flush page
\thispagestyle{empty}
\begin{landscape}

\begin{table}[!t]
        \centering
    \begin{tabular}{|m{0.2\textwidth}<{\centering}|c|c|c|c|c|c|}
    \hline
    Study & Data set & Modality & Preprocessing & Task & Interpretability method & Section \\
    \hline
    \hline
    \cite{abrolDeepResidualLearning2020} & ADNI & T1w & \makecell{GM Segmentation \\ Space registration \\ Smoothing} & AD classification & \makecell{FM visualization \\ Perturbation} & \ref{sec:application_weights_FM}, \ref{sec:application_peturbation}\\
    \hline
    \cite{baeTransferLearningPredicting2019} & ADNI & sMRI & \makecell{Skull stripping \\ Global space registration} & AD classification & Perturbation & \ref{sec:application_peturbation} \\
    \hline
    \cite{ballIndividualVariationUnderlying2020} & PING & T1w & \makecell{Vertex-wise maps (Freesurfer) \\ Spherical registration \\ Smoothing} & Age prediction & \makecell{Weights visualization \\ SHAP} & \ref{sec:application_weights_FM}, \ref{sec:application_distillation} \\
    \hline
    \cite{biffiExplainableAnatomicalShape2020} & ADNI & T1w & \makecell{Hippocampus segmentation \\ Global space registration \\ Upsample + Crop + Pad} & AD classification & FM visualization & \ref{sec:application_weights_FM} \\
    \hline
    \cite{bohleLayerwiseRelevancePropagation2019} & ADNI & T1w & Local space registation & AD classification & \makecell{LRP \\ Guided BP} & \ref{sec:application_BP} \\
    \hline
    \cite{burdujaAccurateEfficientIntracranial2020} & RSNA & CT scan & \makecell{Intensity windows extraction \\ Resizing \\ Intensity normalization} & \makecell{Intracranial Hemorrhage \\ detection} & Grad-CAM & \ref{sec:application_BP} \\
    \hline
    \cite{cecottiConvolutionalNeuralNetworks2011} & in-house & EEG & P300 detection & Weights visualization & \ref{sec:application_weights} \\
    \hline
    \cite{dyrbaComparisonCNNVisualization2020} & ADNI & T1w & \makecell{Tissue segmentation \\ Local space registration \\ Covariates correction} & AD classification & \makecell{DeconvNet \\ DT Decomposition \\ Gradient $\odot$ Input \\ LRP \\ Grad-CAM} & \ref{sec:application_BP} \\
    \hline
    \cite{eitelTestingRobustnessAttribution2019} & ADNI & T1w & Local space registration & AD classification & \makecell{Gradient $\odot$ Input \\ Guided BP \\ LRP \\ Perturbation} & \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    \cite{eitelUncoveringConvolutionalNeural2019} & \makecell{ADNI, \\ in-house} & T1w & \makecell{Global space registration \\ Intensity normalization \\ Tissue segmentation \\ Downsampling + Scaling} & \makecell{Multiple Sclerosis \\ detection} & \makecell{Gradient $\odot$ Input \\ LRP} & \ref{sec:application_BP} \\
    \hline
    
    \end{tabular}
\end{table}

\end{landscape}
\clearpage% Flush page
}

\afterpage{%
\clearpage% Flush page
\thispagestyle{empty}
\begin{landscape}

\begin{table}[!t]
        \centering
    \begin{tabular}{|m{0.2\textwidth}<{\centering}|c|c|c|c|c|c|}
    \hline
    Study & Data set & Modality & Preprocessing & Task & Interpretability method & Section \\
    \hline
    \hline
    \cite{fuAttentionbasedFullSlice2021} & CQ500, RSNA & CT scan & & \makecell{Detection of Critical \\ Findings in Head \\ CT scan} & Attention mechanism & \ref{sec:application_intrinsic} \\
    \hline
    %\cite{fuMeNDTNeuralbackedDecision2021} & RSNA & CT scan & & \makecell{Intracranial Hemorrhage \\ detection} & \makecell{Neural-backed \\ Decision Tree} & \ref{sec:application_distillation} \\
    %\hline
    \cite{gutierrez-beckerDeepMultistructuralShape2018} & ADNI & T1w & Point clouds extraction & AD classification & perturbation & \ref{sec:application_peturbation} \\
    \hline
    \cite{huDeepLearningBasedClassification2021} & ADNI, NIFD & T1w & \makecell{Resample + Crop \\ Intensity normalization} & \makecell{AD/CN/FTD \\ classification} & Guided BP & \ref{sec:application_BP} \\
    \hline
    \cite{jinGeneralizableReproducibleNeuroscientifically2020} & \makecell{ADNI, \\ in-house} & T1w & \makecell{Tissue segmentation \\ Global space registration} & AD classification & Attention mechanism & \ref{sec:application_intrinsic} \\
    \hline
    \cite{leeInterpretableAlzheimerDisease2019} & ADNI & T1w & \makecell{Tissue segmentation \\ Parcellation} & AD classification & Modular transparency & \ref{sec:application_intrinsic} \\
    \hline
    \cite{lemingEnsembleDeepLearning2020} & \makecell{OpenFMRI, ADNI,  \\ ABIDE, ABIDE II, \\ ABCD, NDAR \\ ICBM, UK Biobank, \\ 1000FC} & fMRI & \makecell{Skull-stripping \\ Motion correlation \\ Local space registration \\ Connectivity matrices \\ transformation} & \makecell{Autism classification \\ Sex classification \\ Task vs rest classification} & \makecell{FM visualisation \\ Grad-CAM} & \ref{sec:application_weights_FM}, \ref{sec:application_BP} \\
    \hline
    \cite{martinez-murciaStudyingManifoldStructure2020} & ADNI & T1w & \makecell{Local space registration \\ GM \& WM segmentation \\ Downsampling \\ Intensity normalization} & \makecell{AD classification \\ Prediction of neuro-\\psychological tests \\ \& other clinical variables} & FM visualization & \ref{sec:application_weights_FM} \\
    \hline
    \cite{nigriExplainableDeepCNNs2020} & ADNI, AIBL & T1w & \makecell{Skull-stripping \\ Intensity normalization \\ Global space registration \\ Cropping} & AD classification & \makecell{Perturbation \\ Swap Test} & \ref{sec:application_peturbation} \\
    \hline
    
    \end{tabular}
\end{table}

\end{landscape}
\clearpage% Flush page
}

\afterpage{%
\clearpage% Flush page
\thispagestyle{empty}
\begin{landscape}

\begin{table}[!t]
        \centering
    \begin{tabular}{|m{0.2\textwidth}<{\centering}|c|c|c|c|c|c|}
    \hline
    Study & Data set & Modality & Preprocessing & Task & Interpretability method & Section \\
    \hline
    \hline
    \cite{ohClassificationVisualizationAlzheimer2019} & ADNI & T1w & \makecell{Local space registration \\ Rescaling \\ Intensity normalization} & AD classification & \makecell{FM visualization \\ Standard BP \\ Perturbation} & \ref{sec:application_weights_FM}, \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    \cite{qiuDevelopmentValidationInterpretable2020} & \makecell{ADNI, AIBL, \\ FHS, NACC} & T1w & \makecell{Global space registration \\ Intensity normalization} & AD classification & Modular transparency & \ref{sec:application_intrinsic} \\
    \hline
    \cite{riekeVisualizingConvolutionalNetworks2018} & ADNI & T1w & Local space registration & AD classification & \makecell{Standard BP \\ Guided BP \\ Perturbation \\ Brain Area Occlusion} & \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    \cite{tangInterpretableClassificationAlzheimer2019} & \makecell{UCD-ADC \\ Brain Bank} & histology & Slice color normalization & \makecell{Detection of \\ amyloid-$\beta$ morphologies} & \makecell{Guided BP \\ Perturbation} & \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    \end{tabular}

    \caption{Summary of the presented in Section~\ref{sec:section3}.\\
    \textbf{Data sets}: 1000FC, 1000 Functional Connectomes; ABCD, Adolescent Brain Cognitive Development; ABIDE, Autism Brain Imaging Data Exchange; ADNI, Alzheimer’s Disease Neuroimaging Initiative; AIBL, Australian Imaging, Biomarkers and Lifestyle; FHS, Framingham Heart Study; ICBM, International Consortium for Brain Mapping; NACC, National Alzheimer’s Coordinating Center; NDAR, National Database for Autism Research; NIFD, frontotemporal lobar degeneration neuroimaging initiative; PING, Pediatric Imaging, Neurocognition and Genetics; RSNA, Radiological Society of North America 2019 Brain CT Hemorrhage dataset; UCD-ADC Brain Bank, University of California Davis Alzheimer’s Disease Center Brain Bank. \\
    \textbf{Modalities}: CT, Computed tomography; EEG, Electroencephalography; fMRI, functional Magnetic Resonance Imaging; sMRI, structural Magnetic Resonance Imaging; T1w, T1-weighted [Magnetic Resonance Imaging]. \\
    \textbf{Tasks}: AD, Alzheimer's Disease; CN, Cognitively Normal; FTD, Fronto-Temporal Dementia; MCI, Mild Cognitive Impairment. \\
    \textbf{Interpretability methods}: FM, Feature Maps; Grad-CAM, Gradient-weighted class activation mapping; LRP, Layer-Wise Relevance; SHAP, SHapley Additive exPlanations}
\label{tab:section3}
\end{table}

\end{landscape}
\clearpage% Flush page
}


==> Interpretability Chapter/studies_table_wo_preprocessing.tex <==
\afterpage{%
\clearpage% Flush page
\thispagestyle{empty}
\begin{landscape}

\begin{table}[!t]
    \centering
    \caption[Summary of the studies applying interpretability methods to neuroimaging data]{Summary of the studies applying interpretability methods to neuroimaging data which are presented in Section~\ref{sec:section3}.}
    \label{tab:section3}

    \begin{tabular}{|m{0.35\textwidth}<{\centering}|m{0.25\textwidth}<{\centering}|m{0.15\textwidth}<{\centering}|m{0.3\textwidth}<{\centering}|m{0.4\textwidth}<{\centering}|m{0.1\textwidth}<{\centering}|}
    \hline
    Study & Data set & Modality & Task & Interpretability method & Section \\
    \hline
    \hline
    Abrol et al., 2020~\cite{abrolDeepResidualLearning2020} & ADNI & T1w & AD classification & \makecell{FM visualization \\ Perturbation} & \ref{sec:application_FM}, \ref{sec:application_peturbation}\\
    \hline
    Bae et al., 2019~\cite{baeTransferLearningPredicting2019} & ADNI & sMRI & AD classification & Perturbation & \ref{sec:application_peturbation} \\
    \hline
    Ball et al., 2020~\cite{ballIndividualVariationUnderlying2020} & PING & T1w & Age prediction & \makecell{Weight visualization \\ SHAP} & \ref{sec:application_weights}, \ref{sec:application_distillation} \\
    \hline
    Biffi et al., 2020~\cite{biffiExplainableAnatomicalShape2020} & ADNI & T1w & AD classification & FM visualization & \ref{sec:application_FM} \\
    \hline
    B\"{o}hle et al., 2019~\cite{bohleLayerwiseRelevancePropagation2019} & ADNI & T1w & AD classification & \makecell{LRP \\ Guided back-propagation} & \ref{sec:application_BP} \\
    \hline
    Burduja et al., 2020~\cite{burdujaAccurateEfficientIntracranial2020} & RSNA & CT scan & Intracranial Hemorrhage detection & Grad-CAM & \ref{sec:application_BP} \\
    \hline
    Cecotti and Gr\"{a}ser, 2011~\cite{cecottiConvolutionalNeuralNetworks2011} & in-house & EEG & P300 signals detection & Weight visualization & \ref{sec:application_weights} \\
    \hline
    Dyrba et al., 2020~\cite{dyrbaComparisonCNNVisualization2020} & ADNI & T1w & AD classification & \makecell{DeconvNet \\ Deep Taylor decomposition \\ Gradient $\odot$ Input \\ LRP \\ Grad-CAM} & \ref{sec:application_BP} \\
    \hline
    Eitel and Ritter, 2019~\cite{eitelTestingRobustnessAttribution2019} & ADNI & T1w & AD classification & \makecell{Gradient $\odot$ Input \\ Guided back-propagation \\ LRP \\ Perturbation} & \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    Eitel et al., 2019~\cite{eitelUncoveringConvolutionalNeural2019} & ADNI,  in-house & T1w & Multiple Sclerosis detection & \makecell{Gradient $\odot$ Input \\ LRP} & \ref{sec:application_BP} \\
    \hline
    
    \end{tabular}
\end{table}

\end{landscape}
\clearpage% Flush page
}

\afterpage{%
\clearpage% Flush page
\thispagestyle{empty}
\begin{landscape}

\begin{table}[!t]
        \centering
    \begin{tabular}{|m{0.35\textwidth}<{\centering}|m{0.25\textwidth}<{\centering}|m{0.15\textwidth}<{\centering}|m{0.3\textwidth}<{\centering}|m{0.4\textwidth}<{\centering}|m{0.1\textwidth}<{\centering}|}
    \hline
    Study & Data set & Modality & Task & Interpretability method & Section \\
    \hline
    \hline
    Fu et al., 2021~\cite{fuAttentionbasedFullSlice2021} & CQ500, RSNA & CT scan & Detection of Critical Findings in Head CT scan & Attention mechanism & \ref{sec:application_intrinsic} \\
    \hline
    %\cite{fuMeNDTNeuralbackedDecision2021} & RSNA & CT scan & Intracranial Hemorrhage detection & \makecell{Neural-backed \\ Decision Tree} & \ref{sec:application_distillation} \\
    %\hline
    Guti\'{e}rrez-Becker and Wachinger, 2018~\cite{gutierrez-beckerDeepMultistructuralShape2018} & ADNI & T1w & AD classification & Perturbation & \ref{sec:application_peturbation} \\
    \hline
    Hu et al., 2021~ \cite{huDeepLearningBasedClassification2021} & ADNI, NIFD & T1w & AD/CN/FTD classification & Guided back-propagation & \ref{sec:application_BP} \\
    \hline
    Jin et al., 2020~\cite{jinGeneralizableReproducibleNeuroscientifically2020} & ADNI, in-house & T1w & AD classification & Attention mechanism & \ref{sec:application_intrinsic} \\
    \hline
    Lee et al., 2019~\cite{leeInterpretableAlzheimerDisease2019} & ADNI & T1w & AD classification & Modular transparency & \ref{sec:application_intrinsic} \\
    \hline
    Leming et al., 2020~\cite{lemingEnsembleDeepLearning2020} & OpenFMRI, ADNI, ABIDE, ABIDE II, ABCD, NDAR ICBM, UK Biobank, 1000FC & fMRI & Autism~classification Sex~classification Task~vs~rest classification & \makecell{FM visualization \\ Grad-CAM} & \ref{sec:application_FM}, \ref{sec:application_BP} \\
    \hline
    Magesh et al., 2020~\cite{mageshExplainableMachineLearning2020} & PPMI & SPECT & Parkinson's disease detection & LIME & \ref{sec:application_distillation} \\
    \hline
    Martinez-Murcia et al., 2020~\cite{martinez-murciaStudyingManifoldStructure2020} & ADNI & T1w & AD~classification Prediction~of neuropsychological tests \& other clinical variables & FM visualization & \ref{sec:application_FM} \\
    \hline
    Nigri et al., 2020~\cite{nigriExplainableDeepCNNs2020} & ADNI, AIBL & T1w & AD classification & \makecell{Perturbation \\ Swap test} & \ref{sec:application_peturbation} \\
    \hline
    Oh et al., 2019~\cite{ohClassificationVisualizationAlzheimer2019} & ADNI & T1w & AD classification & \makecell{FM visualization \\ Standard back-propagation \\ Perturbation} & \ref{sec:application_FM}, \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    
    \end{tabular}
\end{table}

\end{landscape}
\clearpage% Flush page
}


\afterpage{%
\clearpage% Flush page
\thispagestyle{empty}
\begin{landscape}

\begin{table}[!t]
    {\centering
    \begin{tabular}{|m{0.35\textwidth}<{\centering}|m{0.25\textwidth}<{\centering}|m{0.15\textwidth}<{\centering}|m{0.3\textwidth}<{\centering}|m{0.4\textwidth}<{\centering}|m{0.1\textwidth}<{\centering}|}
    \hline
    Study & Data set & Modality & Task & Interpretability method & Section \\
    \hline
    \hline
    Qiu et al., 2020~\cite{qiuDevelopmentValidationInterpretable2020} & ADNI, AIBL, FHS, NACC & T1w & AD classification & Modular transparency & \ref{sec:application_intrinsic} \\
    \hline
    Ravi et al., 2022~\cite{raviDegenerativeAdversarialNeuroimage2022} & ADNI & T1w & CN/MCI/AD reconstruction & Modular transparency & \ref{sec:application_intrinsic} \\
    \hline
    Rieke et al., 2018~\cite{riekeVisualizingConvolutionalNetworks2018} & ADNI & T1w & AD classification & \makecell{Standard back-propagation \\ Guided back-propagation \\ Perturbation \\ Brain area occlusion} & \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    Tang et al., 2019~\cite{tangInterpretableClassificationAlzheimer2019} & UCD-ADC, Brain Bank & Histology & Detection of  amyloid-$\beta$ pathology & \makecell{Guided back-propagation \\ Perturbation} & \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    Wood et al., 2019~\cite{woodNEURODRAM3DRecurrent2019} & ADNI & T1w & AD classification & Modular transparency & \ref{sec:application_intrinsic} \\
    \hline
    \end{tabular}
    }

    \bigskip
    \textbf{Data sets}: 1000FC, 1000 Functional Connectomes; ABCD, Adolescent Brain Cognitive Development; ABIDE, Autism Brain Imaging Data Exchange; ADNI, Alzheimer’s Disease Neuroimaging Initiative; AIBL, Australian Imaging, Biomarkers and Lifestyle; FHS, Framingham Heart Study; ICBM, International Consortium for Brain Mapping; NACC, National Alzheimer’s Coordinating Center; NDAR, National Database for Autism Research; NIFD, frontotemporal lobar degeneration neuroimaging initiative; PING, Pediatric Imaging, Neurocognition and Genetics; PPMI, Parkinson’s Progression Markers Initiative; RSNA, Radiological Society of North America 2019 Brain CT Hemorrhage dataset; UCD-ADC Brain Bank, University of California Davis Alzheimer’s Disease Center Brain Bank. \\
    \textbf{Modalities}: CT, computed tomography; EEG, electroencephalography; fMRI, functional magnetic resonance imaging; sMRI, structural magnetic resonance imaging; SPECT,
    single-photon emission computed tomography; T1w, T1-weighted [magnetic resonance imaging]. \\
    \textbf{Tasks}: AD, Alzheimer's disease; CN, cognitively normal; FTD, fronto-temporal dementia; MCI, mild cognitive impairment. \\
    \textbf{Interpretability methods}: FM, feature maps; Grad-CAM, gradient-weighted class activation mapping; LIME, local interpretable model-agnostic explanations; LRP, layer-wise relevance; SHAP, SHapley Additive exPlanations.
\end{table}

\end{landscape}
\clearpage% Flush page
}


==> studies_table.tex <==
\afterpage{%
\clearpage% Flush page
\thispagestyle{empty}
\begin{landscape}

\begin{table}[!t]
        \centering
    \begin{tabular}{|m{0.2\textwidth}<{\centering}|c|c|c|c|c|c|}
    \hline
    Study & Data set & Modality & Preprocessing & Task & Interpretability method & Section \\
    \hline
    \hline
    \cite{abrolDeepResidualLearning2020} & ADNI & T1w & \makecell{GM Segmentation \\ Space registration \\ Smoothing} & AD classification & \makecell{FM visualization \\ Perturbation} & \ref{sec:application_weights_FM}, \ref{sec:application_peturbation}\\
    \hline
    \cite{baeTransferLearningPredicting2019} & ADNI & sMRI & \makecell{Skull stripping \\ Global space registration} & AD classification & Perturbation & \ref{sec:application_peturbation} \\
    \hline
    \cite{ballIndividualVariationUnderlying2020} & PING & T1w & \makecell{Vertex-wise maps (Freesurfer) \\ Spherical registration \\ Smoothing} & Age prediction & \makecell{Weights visualization \\ SHAP} & \ref{sec:application_weights_FM}, \ref{sec:application_distillation} \\
    \hline
    \cite{biffiExplainableAnatomicalShape2020} & ADNI & T1w & \makecell{Hippocampus segmentation \\ Global space registration \\ Upsample + Crop + Pad} & AD classification & FM visualization & \ref{sec:application_weights_FM} \\
    \hline
    \cite{bohleLayerwiseRelevancePropagation2019} & ADNI & T1w & Local space registation & AD classification & \makecell{LRP \\ Guided BP} & \ref{sec:application_BP} \\
    \hline
    \cite{burdujaAccurateEfficientIntracranial2020} & RSNA & CT scan & \makecell{Intensity windows extraction \\ Resizing \\ Intensity normalization} & \makecell{Intracranial Hemorrhage \\ detection} & Grad-CAM & \ref{sec:application_BP} \\
    \hline
    \cite{cecottiConvolutionalNeuralNetworks2011} & in-house & EEG & P300 detection & Weights visualization & \ref{sec:application_weights} \\
    \hline
    \cite{dyrbaComparisonCNNVisualization2020} & ADNI & T1w & \makecell{Tissue segmentation \\ Local space registration \\ Covariates correction} & AD classification & \makecell{DeconvNet \\ DT Decomposition \\ Gradient $\odot$ Input \\ LRP \\ Grad-CAM} & \ref{sec:application_BP} \\
    \hline
    \cite{eitelTestingRobustnessAttribution2019} & ADNI & T1w & Local space registration & AD classification & \makecell{Gradient $\odot$ Input \\ Guided BP \\ LRP \\ Perturbation} & \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    \cite{eitelUncoveringConvolutionalNeural2019} & \makecell{ADNI, \\ in-house} & T1w & \makecell{Global space registration \\ Intensity normalization \\ Tissue segmentation \\ Downsampling + Scaling} & \makecell{Multiple Sclerosis \\ detection} & \makecell{Gradient $\odot$ Input \\ LRP} & \ref{sec:application_BP} \\
    \hline
    
    \end{tabular}
\end{table}

\end{landscape}
\clearpage% Flush page
}

\afterpage{%
\clearpage% Flush page
\thispagestyle{empty}
\begin{landscape}

\begin{table}[!t]
        \centering
    \begin{tabular}{|m{0.2\textwidth}<{\centering}|c|c|c|c|c|c|}
    \hline
    Study & Data set & Modality & Preprocessing & Task & Interpretability method & Section \\
    \hline
    \hline
    \cite{fuAttentionbasedFullSlice2021} & CQ500, RSNA & CT scan & & \makecell{Detection of Critical \\ Findings in Head \\ CT scan} & Attention mechanism & \ref{sec:application_intrinsic} \\
    \hline
    %\cite{fuMeNDTNeuralbackedDecision2021} & RSNA & CT scan & & \makecell{Intracranial Hemorrhage \\ detection} & \makecell{Neural-backed \\ Decision Tree} & \ref{sec:application_distillation} \\
    %\hline
    \cite{gutierrez-beckerDeepMultistructuralShape2018} & ADNI & T1w & Point clouds extraction & AD classification & perturbation & \ref{sec:application_peturbation} \\
    \hline
    \cite{huDeepLearningBasedClassification2021} & ADNI, NIFD & T1w & \makecell{Resample + Crop \\ Intensity normalization} & \makecell{AD/CN/FTD \\ classification} & Guided BP & \ref{sec:application_BP} \\
    \hline
    \cite{jinGeneralizableReproducibleNeuroscientifically2020} & \makecell{ADNI, \\ in-house} & T1w & \makecell{Tissue segmentation \\ Global space registration} & AD classification & Attention mechanism & \ref{sec:application_intrinsic} \\
    \hline
    \cite{leeInterpretableAlzheimerDisease2019} & ADNI & T1w & \makecell{Tissue segmentation \\ Parcellation} & AD classification & Modular transparency & \ref{sec:application_intrinsic} \\
    \hline
    \cite{lemingEnsembleDeepLearning2020} & \makecell{OpenFMRI, ADNI,  \\ ABIDE, ABIDE II, \\ ABCD, NDAR \\ ICBM, UK Biobank, \\ 1000FC} & fMRI & \makecell{Skull-stripping \\ Motion correlation \\ Local space registration \\ Connectivity matrices \\ transformation} & \makecell{Autism classification \\ Sex classification \\ Task vs rest classification} & \makecell{FM visualisation \\ Grad-CAM} & \ref{sec:application_weights_FM}, \ref{sec:application_BP} \\
    \hline
    \cite{martinez-murciaStudyingManifoldStructure2020} & ADNI & T1w & \makecell{Local space registration \\ GM \& WM segmentation \\ Downsampling \\ Intensity normalization} & \makecell{AD classification \\ Prediction of neuro-\\psychological tests \\ \& other clinical variables} & FM visualization & \ref{sec:application_weights_FM} \\
    \hline
    \cite{nigriExplainableDeepCNNs2020} & ADNI, AIBL & T1w & \makecell{Skull-stripping \\ Intensity normalization \\ Global space registration \\ Cropping} & AD classification & \makecell{Perturbation \\ Swap Test} & \ref{sec:application_peturbation} \\
    \hline
    
    \end{tabular}
\end{table}

\end{landscape}
\clearpage% Flush page
}

\afterpage{%
\clearpage% Flush page
\thispagestyle{empty}
\begin{landscape}

\begin{table}[!t]
        \centering
    \begin{tabular}{|m{0.2\textwidth}<{\centering}|c|c|c|c|c|c|}
    \hline
    Study & Data set & Modality & Preprocessing & Task & Interpretability method & Section \\
    \hline
    \hline
    \cite{ohClassificationVisualizationAlzheimer2019} & ADNI & T1w & \makecell{Local space registration \\ Rescaling \\ Intensity normalization} & AD classification & \makecell{FM visualization \\ Standard BP \\ Perturbation} & \ref{sec:application_weights_FM}, \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    \cite{qiuDevelopmentValidationInterpretable2020} & \makecell{ADNI, AIBL, \\ FHS, NACC} & T1w & \makecell{Global space registration \\ Intensity normalization} & AD classification & Modular transparency & \ref{sec:application_intrinsic} \\
    \hline
    \cite{riekeVisualizingConvolutionalNetworks2018} & ADNI & T1w & Local space registration & AD classification & \makecell{Standard BP \\ Guided BP \\ Perturbation \\ Brain Area Occlusion} & \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    \cite{tangInterpretableClassificationAlzheimer2019} & \makecell{UCD-ADC \\ Brain Bank} & histology & Slice color normalization & \makecell{Detection of \\ amyloid-$\beta$ morphologies} & \makecell{Guided BP \\ Perturbation} & \ref{sec:application_BP}, \ref{sec:application_peturbation} \\
    \hline
    \end{tabular}

    \caption{Summary of the presented in Section~\ref{sec:section3}.\\
    \textbf{Data sets}: 1000FC, 1000 Functional Connectomes; ABCD, Adolescent Brain Cognitive Development; ABIDE, Autism Brain Imaging Data Exchange; ADNI, Alzheimer’s Disease Neuroimaging Initiative; AIBL, Australian Imaging, Biomarkers and Lifestyle; FHS, Framingham Heart Study; ICBM, International Consortium for Brain Mapping; NACC, National Alzheimer’s Coordinating Center; NDAR, National Database for Autism Research; NIFD, frontotemporal lobar degeneration neuroimaging initiative; PING, Pediatric Imaging, Neurocognition and Genetics; RSNA, Radiological Society of North America 2019 Brain CT Hemorrhage dataset; UCD-ADC Brain Bank, University of California Davis Alzheimer’s Disease Center Brain Bank. \\
    \textbf{Modalities}: CT, Computed tomography; EEG, Electroencephalography; fMRI, functional Magnetic Resonance Imaging; sMRI, structural Magnetic Resonance Imaging; T1w, T1-weighted [Magnetic Resonance Imaging]. \\
    \textbf{Tasks}: AD, Alzheimer's Disease; CN, Cognitively Normal; FTD, Fronto-Temporal Dementia; MCI, Mild Cognitive Impairment. \\
    \textbf{Interpretability methods}: FM, Feature Maps; Grad-CAM, Gradient-weighted class activation mapping; LRP, Layer-Wise Relevance; SHAP, SHapley Additive exPlanations}
\label{tab:section3}
\end{table}

\end{landscape}
\clearpage% Flush page
}

